Dress-Me-Up: A Dataset & Method for Self-Supervised 3D Garment Retargeting

We propose a novel self-supervised framework for retargeting non-parameterized 3D garments onto 3D human avatars of arbitrary shapes and poses, enabling 3D virtual try-on (VTON). Existing self-supervised 3D retargeting methods only support parametric and canonical garments, which can only be draped over parametric body, e.g. SMPL. To facilitate the non-parametric garments and body, we propose a novel method that introduces Isomap Embedding based correspondences matching between the garment and the human body to get a coarse alignment between the two meshes. We perform neural refinement of the coarse alignment in a self-supervised setting. Further, we leverage a Laplacian detail integration method for preserving the inherent details of the input garment. For evaluating our 3D non-parametric garment retargeting framework, we propose a dataset of 255 real-world garments with realistic noise and topological deformations. The dataset contains $44$ unique garments worn by 15 different subjects in 5 distinctive poses, captured using a multi-view RGBD capture setup. We show superior retargeting quality on non-parametric garments and human avatars over existing state-of-the-art methods, acting as the first-ever baseline on the proposed dataset for non-parametric 3D garment retargeting.

==> figures/references/0_teaser.tex <==
%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
\twocolumn[{%
    \renewcommand\twocolumn[1][]{#1}%
    \maketitle
    \begin{center}
        %\centering
        \includegraphics[width=\linewidth]{figures/teaser.pdf}
        \captionof{figure}{3D garment retargeting on real human scans using our approach (left) and our real 3D garment dataset samples(right).}
        \label{fig:teaser}
    \end{center}%
}]


==> figures/references/10_dino_features.tex <==
\begin{figure*}
    \centering
    \rotatebox[origin=c]{90}{Teacher DINO\Bstrut}
    \rotatebox[origin=c]{90}{(\garden)\Bstrut}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/teacher/0.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/teacher/1.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/teacher/2.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/teacher/3.png}}
    \end{minipage}
    
    \rotatebox[origin=c]{90}{Distilled\Bstrut}
    \rotatebox[origin=c]{90}{(\garden)\Bstrut}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/student/0.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/student/1.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/student/2.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/garden/student/3.png}}
    \end{minipage}
    
    % kitchen
    \rotatebox[origin=c]{90}{Teacher DINO\Bstrut}
    \rotatebox[origin=c]{90}{(\kitchen)\Bstrut}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/teacher/0.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/teacher/1.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/teacher/2.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/teacher/3.png}}
    \end{minipage}
    
    \rotatebox[origin=c]{90}{Distilled\Bstrut}
    \rotatebox[origin=c]{90}{(\kitchen)\Bstrut}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/student/0.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/student/1.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/student/2.png}}
    \end{minipage}
    \begin{minipage}{0.23\linewidth}
        \centering
        {\includegraphics[width=\textwidth, height=3cm]{assets/images/dino_features/kitchen/student/3.png}}
    \end{minipage}
    
    \caption{\emph{Student Surpasses Teacher}:
    {The 4 columns of this figure shows the DINO features used as teacher vs the ones learnt by student post optimization. Since, the student learns finer features than the teacher due to assistance from the volumetric density, we can claim that the student surpasses the teacher. This is consistent with the prior art N3F and DFF}}
    \label{fig:dino_features}
\end{figure*}

==> figures/references/11_all_n3f.tex <==
\begin{figure*}
    \centering
    % garden
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/chesstable/0.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/colorfountain/0.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/stove/0.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/shoerack/0.png}}
    \end{minipage}
    
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/chesstable/1.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/colorfountain/1.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/stove/1.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/shoerack/1.png}}
    \end{minipage}
    
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/chesstable/2.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/colorfountain/2.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/stove/2.png}}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/shoerack/2.png}}
    \end{minipage}
    
    \begin{minipage}{0.24\linewidth}
    \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/chesstable/3.png}}
        \subcaption{\chesstable}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
    \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/colorfountain/3.png}}
        \subcaption{\colorfountain}
    % \subcaptionbox{\colorfountain}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
    \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/stove/3.png}}
        \subcaption{\stove}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
    \centering
        \frame{\includegraphics[width=\textwidth, height=3cm]{assets/images/all_n3f/shoerack/3.png}}
        \subcaption{\shoerack}
    % \subcaptionbox{\shoerack}
    \end{minipage}
    \caption{\emph{N3F/DFF Results}:
    {In this figure we show result of DFF and N3F on different thresholds and in the main document we provided the best of their method. Here, we display the segmentation obtained by N3F/DFF \cite{N3F}. It can be seen that despite varying the thresholds the result is poorly segmented. The background objects are starting to bleed into the foreground. For the results of our method on the same scenes, please refer to the main paper.}}
    \label{fig:all_n3f}
\end{figure*}

==> figures/references/3_joint_mask.tex <==
% \begin{figure*}
%     \centering
%     \begin{minipage}{0.24\linewidth}
%         \centering
%         \subcaptionbox{Rendered Image}{\includegraphics[width=\textwidth, height=3cm]{assets/images/growing/gt_cropped.png}}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \centering
%         \subcaptionbox{High Confidence Region}{\includegraphics[width=\textwidth, height=3cm]{assets/images/growing/nnfm_cropped.png}}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \centering
%         \subcaptionbox{Iteration 1}{\includegraphics[width=\textwidth, height=3cm]{assets/images/growing/iter1_cropped.png}}
%     \end{minipage}
%     \begin{minipage}{0.24\linewidth}
%         \centering
%         \subcaptionbox{Iteration 2}{\includegraphics[width=\textwidth, height=3cm]{assets/images/growing/iter2_cropped.png}}
%     \end{minipage}
%     \caption{\emph{Region Growing}:
%     {Image (a) is the reference rendered viewpoint. Image (b) is the high confidence region which misses out frontal region of the dry-leaf when extracting the content. Image (c) shows the result obtained after the first iteration of bilateral search, which captures most of the desired region of the leaf. Image (d) is the result of the bilateral search applied for the second time to include intricate details such as strands around the dry-leaf.}}
%     \label{fig:bilateral_growth}
% \end{figure*}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/joints.png}
  \caption{Joint mask loss} 
\label{fig:joint_mask}
\end{figure}

==> figures/references/5_m3dvton.tex <==
\begin{figure}
    \centering    
    \begin{minipage}{0.44\linewidth}
        \centering
        \subcaptionbox{Garment}{{
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/m3dvton/inp_garment.png}};
        \end{tikzpicture}
        }}
    \end{minipage}
    \begin{minipage}{0.44\linewidth}
        \centering
        \subcaptionbox{Desired-pose}{{
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/m3dvton/inp_pose.png}};
        \end{tikzpicture}
        }}
    \end{minipage}
    \begin{minipage}{0.44\linewidth}
        \centering
        \subcaptionbox{M3DVTON}{{
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/m3dvton/m3dvton.png}};
        \end{tikzpicture}
        }}
    \end{minipage}
   \begin{minipage}{0.44\linewidth}
        \centering
        \subcaptionbox{Ours}{{
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/m3dvton/ours.png}};
        \end{tikzpicture}
        }}
    \end{minipage}
    \caption{Comparison with M3DVTON.}
    \label{fig:m3dvton}\vspace{5mm}
\end{figure}


==> figures/references/6_wrinkle.tex <==
% \begin{figure}
%     \centering
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Stroke 1}
%         {\includegraphics[width=\linewidth]{assets/images/double_positive/gt_stroke1.png}}
%     \end{minipage}
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Output 1}
%          {\includegraphics[width=\linewidth]{assets/images/double_positive/one.png}}
%     \end{minipage}
    
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Stroke 2}
%         {\includegraphics[width=\linewidth]{assets/images/double_positive/gt_stroke2.png}}
%     \end{minipage}
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Merged Output}
%         {\includegraphics[width=\linewidth]{assets/images/double_positive/union.png}}
%     \end{minipage}
%     \caption{\emph{Multiple Positive Strokes}:
%     {When the method fails to capture some of the details using one stroke, the user can add more positive strokes to recover the object of interest. Here, the user makes three strokes in (a). The teeth of the JCB are not extracted well in (b). When the user makes an additional stroke on one of the teeth (c) and the resultant image (d) capture the full details.}}
%     \label{fig:double_positive}
% \end{figure}
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figures/wrinkles.png}
%   \caption{Results of wrinkle generation on unseen garment} 
%   \label{fig:wrinkle}
% \end{figure}

==> figures/references/8_nsim.tex <==
% \begin{figure}
%     \centering
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Rendered View 1}
%          {\includegraphics[width=\linewidth]{assets/images/trex/rendered_0.png}}
%     \end{minipage}
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Rendered View 2}
%          {\includegraphics[width=\linewidth]{assets/images/trex/rendered_1.png}}
%     \end{minipage}
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Segmented Trex}
%          {\includegraphics[width=\linewidth]{assets/images/trex/segmented.png}}
%     \end{minipage}
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \subcaptionbox{Depth Map}
%         {\includegraphics[width=\linewidth]{assets/images/trex/depth.png}}
%     \end{minipage}
    
%     \caption{ \emph{Finer Segmentation}:
%     %{Image (a) shows the rendered output of a radiance field. Image (b) shows our segmented output. We are able to achieve fine-grained segmentation on objects such as the ribcage bones of the T-Rex. However, when observed closely, the region near the tail bleed some background into the foreground. This is due to the dense packing of voxels in forward facing direction. This can be mitigated either by having high resolution voxel grid or more 3D information augmenting the border between the two foreground and background region.}}
%     {Images (a) and (b) show rendered views of T-Rex from the LLFF dataset \cite{mildenhall2019llff}. Image (c) shows the segmented output of T-Rex scene in LLFF dataset. We are able to achieve fine-grained segmentation of objects such as the rib-cage bones of T-Rex. However, when observed closely, the region near the tail bones contains some background as well. This is due to the background and the tail bones lying at the same distance as shown in the depth map (d). This can be mitigated by having more 3D information (better training views) or higher voxel grid resolution.}}
%     \label{fig:trex}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.63\linewidth]{assets/images/sim.png}
    \caption{Neural Cloth Simulation\cite{neural_cloth_sim} results with (a) Jump and (b) Smooth trajectory. }
    \label{fig:NeuralSim}
\end{figure}

==> figures/references/9_steelball.tex <==
\begin{figure*}
    \centering
    \begin{minipage}{0.49\linewidth}
        \centering
        \subcaptionbox{With Steel Balls}{{
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/steelball/with.png}};
            \begin{scope}[x={(image.south east)},y={(image.north west)}]
                \draw[orange,thick] (0.8,0.55) rectangle (1.0, 0.85);
            \end{scope}
        \end{tikzpicture}
        }}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \centering
        \subcaptionbox{Without Steel Balls}{{
        \begin{tikzpicture}
            \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{assets/images/steelball/without.png}};
        \end{tikzpicture}
        }}
    \end{minipage}
    
    \caption{ \emph{Removal of Steel Balls}:
    {DVGO uses a part of MipNeRF360\cite{mipnerf360} formulation in voxel space for unbounded 360 degree scenes. This gives fewer number of voxels to the background objects compared to the central volume of interest. In this scene, we remove the steel balls appearing in the background region of the scene.}}
    \label{fig:stellballs}
\end{figure*}


==> figures/references/detail_transfer.tex <==
\begin{figure} 
\centering
\includegraphics[width=\linewidth]{figures/detail_transfer2_comp.png}
\caption{1} 
\label{fig:detail_transfer2_comp}
\end{figure}
    

==> figures/references/shape_pose.tex <==
\begin{figure} 
\centering
\includegraphics[width=\linewidth]{figures/shape_pose_nonparam.png}
\caption{1} 
\label{fig:cloth3d_amaas_new}
\end{figure}

==> figures/suppl_figures/m3dvton.tex <==
\begin{figure*}
    \begin{tikzpicture}[scale=0.9]
    \node (A) at (-.5,0) {\includegraphics[width=1.05\textwidth]{assets/images/suppl_figures/m3dvton/m3dvton_comp1.png}};
    \node (B) at (0,-10) {\includegraphics[width=\textwidth, trim={0 0 0 12cm},clip]{assets/images/suppl_figures/m3dvton/m3dvton_comp2.png}};
    \end{tikzpicture}
    \caption{The figure shows retargeting results on images of MPV3D\cite{M3DVTON} against the results obtained by M3DVTON. Please observe the geometric inconsistencies in the results of M3DVTON despite having simple garment structures}
    \label{fig:m3dvton}
\end{figure*}



==> figures/suppl_figures/wrinkle_generation_pipeline.tex <==
\begin{figure}
    \includegraphics[width=\linewidth]{assets/images/suppl_figures/wrinkle_generation/wrinkle_gen.png};
    \caption{Pipeline Diagram for Wrinkle generation}
    \label{fig:wrinkle_generation}
\end{figure}

==> imports/1_macros.tex <==
% inset image border color
\fboxsep=0.5mm%padding thickness
\fboxrule=0pt%border thickness


% Add a period to the end of an abbreviation unless there's one already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\def\st{\emph{s.t}\onedot}
\makeatother

% norm
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

% TODOnotes
\newcommandx{\doit}[2][1=]{\todo[linecolor=olive,backgroundcolor=olive!25,bordercolor=olive,#1]{#2}}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=teal,backgroundcolor=teal!25,bordercolor=teal,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}

\newcommand{\AR}[1]{{\color{blue}[\textbf{AR:} #1]}}


\newcommand{\smpl}{\textsc{SMPL}~}
% \newcommand{\sleeveless}{\textsc{SleeveLess}~}
% \newcommand{\sleeved}{\textsc{Sleeved}~}
% \newcommand{\trousers}{\textsc{Trousers}~}
\newcommand{\topwear}{\textsc{TW}~}
\newcommand{\bottomwear}{\textsc{BW}~}

\DeclareMathOperator*{\argminA}{arg\,min} % Jan Hlavacek
\DeclareMathOperator*{\argmaxA}{arg\,max} % Jan Hlavacek

% Define typographic struts, as suggested by Claudio Beccari
%   in an article in TeX and TUG News, Vol. 2, 1993.
\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut

% comment out large regions
\newcommand{\Comments}[1]{}

% Sapcing EDITS
% Consistent margin adjustment for paragraphs, figures, and sections
\newlength\paramargin
\newlength\figmargin
\newlength\secmargin
\newlength\figcapmargin
\newlength\tabcapmargin

% \setlength{\secmargin}{0.0mm}
% \setlength{\paramargin}{0.0mm}
% \setlength{\figmargin}{0.0mm}
% \setlength{\tabcapmargin}{0.0mm}

\newcommand{\Paragraph}[1]
{\vspace{2mm} \noindent \textbf{#1}}

==> imports/2_copyright.tex <==
\def\iccvPaperID{4460} % *** Enter the ICCV Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% Pages are numbered in submission mode, and unnumbered in camera-ready
\ificcvfinal\pagestyle{empty}\fi

% \iccvfinalcopy % *** Uncomment this line for the final submission

==> imports/3_header.tex <==

%%%%%%%%% TITLE
\title{Dress Me Up: A Dataset \& Method for Self-Supervised 3D Garment Retargeting}

\author{First Author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}

==> tables/4_kinect.tex <==
% \begin{table*}[tbh]
%     \centering
%     \begin{tabular}
%     {|p{0.05\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|p{0.05\textwidth}|}
%      \hline
%      \multicolumn{1}{|c|}{Garment Type} & \multicolumn{1}{c|}{P2S} & \multicolumn{1}{c|}{Euclidean} & \multicolumn{1}{c|}{L2norm} & \multicolumn{1}{c|}{Normal Consistancy} \\
%      \hline
%     \multicolumn{1}{|c|}{\sleeveless} & \multicolumn{1}{c|}{ 0.00632} & \multicolumn{1}{c|}{0.00916} & \multicolumn{1}{c|}{0.00026}& \multicolumn{1}{c|}{0.9418}  \\
    
%     \multicolumn{1}{|c|}{\sleeved} & \multicolumn{1}{c|}{0.00748} & \multicolumn{1}{c|}{0.00954} & \multicolumn{1}{c|}{0.00059} & \multicolumn{1}{c|}{0.8379}  \\
    
%     \multicolumn{1}{|c|}{\trousers} & \multicolumn{1}{c|}{0.008049} & \multicolumn{1}{c|}{0.00983} & \multicolumn{1}{c|}{0.000574} & \multicolumn{1}{c|}{0.8882}  \\
     
    
%     \hline
%     \end{tabular}
%     \caption{Loss evaluation on cloth3d dataset}
%     \label{tbl:cloth3d_cd_p2s}
% \end{table*}

% \begin{table}
%     \centering
%     \begin{tabular}
%     {|p{0.18\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|}
%      \hline
%      {Garment Type} & {P2S} & {ED} & {L2N} & {NC} \\
     
%      \hline
%     {\sleeved} & {0.01211} & {0.0125} & {0.01449}  & { -} \\
    
%     {\trousers} & {0.00675} & {0.007314} & { 0.01413}  & {-} \\
    
%     \hline
%     \end{tabular}
%     \caption{\emph{Our real-garment data:} Here we show P2S, Euclidean distance(ED), L2-Norm (L2N) and Normal Consistency (NC) on two garment categories \sleeved and \trousers}
%     \label{tbl:kinect_data}
% \end{table}

==> tables/6_wrinkle_ablation.tex <==

\begin{table}
    \centering
    \begin{tabular}{|l |l l| l|}
    \hline
    \multicolumn{4}{|c|}{\textsc{3DHumans Dataset}} \\
    \hline
    {\textsc{Type}} & {P2S$\downarrow$} & \multicolumn{1}{c|}{ED$\downarrow$} & {NC$\uparrow$} \\
    {}    & \multicolumn{2}{c|}{x $10^{-3}$} &  \\
    \hline
    % \multicolumn{5}{|c|}{}\\
    {\topwear}    & {1.156} & {2.362}  & {0.8447}  \\
    {\bottomwear}   & {0.744} & {1.077}  & {0.945} \\
    \hline
    % \multicolumn{5}{|c|}{}\\
    \multicolumn{4 }{|c|}{\textsc{THuman2.0}}\\
    \hline
    % \multicolumn{5}{|c|}{}\\
   {\topwear} & {1.703} & {2.632}  & { 0.865} \\
    {\bottomwear} & {1.200} & {2.264}  & { 0.9159} \\
    \hline
    \end{tabular}
     \caption{Quantitative evaluation of Wrinkle Generation Network}
    \label{table:wrinkle_tab}
\end{table}

% {\sleeveless} & { 6.3216} & {9.1641} & {0.2609}& {0.9665}  \\
% {\sleeved}    & {7.4813} & {9.5436} & {0.5925} & {0.9343}  \\
% \multicolumn{1}{|c}
% \multicolumn{1}{c|}

